Strong Secrecy in Pairwise Key Agreement over a Generalized Multiple Access Channel

This paper considers the problem of pairwise key agreement without public communication between three users connected through a generalized multiple access channel (MAC). While two users control the channel inputs, all three users observe noisy outputs from the channel and each pair of users wishes to agree on a secret key hidden from the remaining user. We first develop a "pre-generated" key-agreement scheme based on secrecy codes for the generalized MAC, in which the channel is only used to distribute pre-generated secret keys. We then extend this scheme to include an additional layer of rate-limited secret-key generation by treating the observed channel outputs as induced sources. We characterize inner and outer bounds on the strong secret-key capacity region for both schemes. For a special case of the "pre-generated" scheme, we obtain an exact characterization. We also illustrate with some binary examples that exploiting the generalized nature of the generalized MAC may lead to significantly larger key-agreement rates.

==> preliminaries2.tex <==

% in which the key generated from the channel output at the end of each block is sent over the channel in the next block
%In particular, the keys generated by uses 1 and 2 are generally functions of the channel input and outputs.
%We first present the formal definition of the described secret key sharing as shown in Fig. \ref{fig_sim}.

%\noindent{\textit{Step 1})} $n$ uses of the GDMMAC: User 1 generates the $i$th channel input $X_{1,i}$, $i\in[1,..,n]$, as stochastic function of the previous channel outputs $Y_{1}^{i-1}$. User 2 similarly generates $X_{2,i}$ for $i=1,2,...,n$. Subsequently, the outputs $Y_{1,i},Y_{2,i}$ and $Y_{3,i}$ are observed by Users 1, 2, and 3, respectively.
%
%\noindent{\textit{Step 2})} Generation of the respective keys: User 1  generates $K_{12}$ and $K_{13}$ as stochastic functions of $(X_{1}^{n},Y_{1}^{n}\!)$ for sharing with Users 2 and 3, respectively. Similarly, $\hat{K}_{12}$ and $K_{23}$ are generated by User 2 for sharing with Users 1 and 3, respectively, as stochastic functions of $(X_{2}^{n},Y_{2}^{n}\!)$. User 3 also generates $\hat{K}_{13}$ and  $\hat{K}_{23}$ as functions of $Y_{3}^{n}$.
%
%\indent After these steps, $K_{12}$ is shared between Users l and 2, $K_{13}$ between Users 1 and 3, and $K_{23}$ between Users 2 and User 3. All the above keys take values in some finite sets. As in Definition 1, some conditions should be satisfied in the described secret key sharing framework.


%\begin{defi}
%\label{def3}
%In the generalized scheme of the pairwise secret key sharing, the rate triple $(R_{12},R_{13},R_{23})$ is an achievable key rate triple if for every $\varepsilon>0$ and all sufficiently large $n$, we have:
%
%\noindent \begin{align}
%&{{\tfrac{1}{n}}H(K_{12})>R_{12}-\varepsilon,{\tfrac{1}{n}}H(K_{13})>R_{13}-\varepsilon,{\tfrac{1}{n}}H(K_{23})>R_{23}-\varepsilon} \label{eq4}
%\\&{\Pr\{K_{12}\ne \hat{K}_{12}\}<\varepsilon,\Pr\{K_{13}\ne\hat{K}_{13}\}<\varepsilon,\Pr\{K_{23}\ne\hat{K}_{23}\}<\varepsilon} \label{eq5}
%\\&{{\tfrac{1}{n}}I(K_{12};Y_{3}^{n})<\varepsilon,{\tfrac{1}{n}}I(K_{13};X_{2}^{n},Y_{2}^{n})<\varepsilon,{ \tfrac{1}{n}}I(K_{23};X_{1}^{n},Y_{1}^{n})<\varepsilon} \label{eq6}
% \end{align}
%
%Equations (\ref{eq4})-(\ref{eq6}) are justified as Equations (\ref{eq1})-(\ref{eq3}) in Definition \ref{def1} and the secret key capacity region is defined the same as in Definition \ref{def2}. Furthermore, the weak security conditions (\ref{eq6}) can be changed to the strong ones and correspondingly, the strongly secret key capacity region is defined.
%\end{defi}

%the key pair $K_{1,2}=(K_{12},K_{21})$ is shared between user l and user 2, $K_{13}$ between user 1 and User 3, and $K_{23}$ between user 2 and User 3. All the above keys take values in some finite sets. Now, we state the conditions that should be met in the described secret key sharing framework.
%
%\begin{figure}%[!t]
%\centering
%%\vspace{-.4cm}
%\includegraphics[width=9cm]{Drawing1.pdf}
%\vspace{-.3cm}
%\caption{\footnotesize{Secret key sharing over GDMMAC using noiseless feedback channel}}
%\vspace{-.5cm}
%\label{fig_sim}
%\end{figure}
%\begin{defi}
%\label{def1}
%In the pairwise secret key sharing of the proposed model, the rate triple $(R_{12},R_{13},R_{23})$ is an achievable key rate triple if for every $\varepsilon>0$ and sufficiently large $n$, we have:
%
%\noindent \begin{align}
%&{{\tfrac{1}{n}}H(K_{1,2})={\tfrac{1}{n}}H(K_{12},K_{21})>R_{12}-\varepsilon,{\tfrac{1}{n}}H(K_{13})>R_{13}-\varepsilon,{\tfrac{1}{n}}H(K_{23})>R_{23}-\varepsilon} \label{eq1}
%\\&{\Pr\{(K_{12},K_{21})\ne(\hat{K}_{12},\!\hat{K}_{21})\}<\varepsilon,\Pr\{K_{13}\ne\hat{K}_{13}\}<\varepsilon,\Pr\{K_{23}\ne\hat{K}_{23}\}<\varepsilon} \label{eq2}
%\\&{{\tfrac{1}{n}}I(K_{12},K_{21};Y_{3}^{n})<\varepsilon,{\tfrac{1}{n}}I(K_{13};X_{2}^{n},Y_{2}^{n})<\varepsilon,{ \tfrac{1}{n}}I(K_{23};X_{1}^{n},Y_{1}^{n})<\varepsilon} \label{eq3}
% \end{align}
%
%\noindent\normalsize Equation \eqref{eq1} means that the rates $R_{12},R_{13}$ and $R_{23}$ are the rates of the secret keys between users 1 and 2, users 1 and 3, and users 2 and 3, respectively.
%Equation \eqref{eq2} means that each user can correctly estimate the related keys. Equation \eqref{eq3} means that each user effectively has no information about the remaining users' secret key.
%\end{defi}
%\begin{defi}
%\label{def2}
%The region containing all the achievable secret key rate triples $(R_{12},R_{13},R_{23})$ is the secret key capacity region.
%\end{defi}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "game"
%%% End:

